Energy-Based Models for Continual Learning

We motivate Energy-Based Models (EBMs) as a promising model class for continual learning problems. Instead of tackling continual learning via the use of external memory, growing models, or regularization, EBMs change the underlying training objective to cause less interference with previously learned information. Our proposed version of EBMs for continual learning is simple, efficient, and outperforms baseline methods by a large margin on several benchmarks. Moreover, our proposed contrastive divergence-based training objective can be combined with other continual learning methods, resulting in substantial boosts in their performance. We further show that EBMs are adaptable to a more general continual learning setting where the data distribution changes without the notion of explicitly delineated tasks. These observations point towards EBMs as a useful building block for future continual learning methods.

==> text/checklist.tex <==

\section*{Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See Section~\ref{sect:conclusion}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See Section~\ref{sect:conclusion}.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We provided the details in \sect{sec:experiments} and supplemental material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{We provided the details in \sect{sec:experiments} and supplemental material.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{All the experiments reported in \sect{sec:experiments} use multiple random seeds. The mean and standard error of the mean are reported in each table.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See supplemental material.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}



==> text/figures_new/confusion.tex <==
\begin{figure}[h]
\begin{center}
\includegraphics[width=0.8\textwidth]{text/figures_new/files/split_confusion.pdf}
\end{center}
\vspace{-5pt}
\caption{\small Confusion matrices between ground truth labels and predicted labels at the end of learning on split MNIST (left) and permuted MNIST (right). The lighter the diagonal is, the more accurate the predictions are.}
\label{fig:new_confusion_matrix}
\end{figure} 

==> text/figures_new/confusion_label_distributation.tex <==
\begin{figure}[h]
     \centering
     \begin{minipage}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=0.9\textwidth]{text/figures_new/files/split_label_distributation.pdf}
         \vspace{-10pt}
         \caption{\small Predicted label distribution after learning each task on the split MNIST dataset. 
         CLS only predict classes from the current task while EBMs can predict classes for all seen classes.
        %   The more uniform the distribution is, the better the model is in preventing forgetting previous tasks.
        }
        \label{fig:new_label_distributation}
     \end{minipage}
     \hfill
     \begin{minipage}[b]{0.52\textwidth}
         \centering
         \includegraphics[width=1\textwidth]{text/figures_new/files/split_confusion.pdf}
         \vspace{-20pt}
        \caption{\small Confusion matrices between ground truth labels and predicted labels at the end of learning on split MNIST (left) and permuted MNIST (right). The lighter the diagonal is, the more accurate the predictions are.}
        \label{fig:new_confusion_matrix}
    \end{minipage}
\end{figure}

==> text/figures_new/fisher.tex <==
\begin{figure}
\begin{center}
% \includegraphics[width=1\linewidth]{text/figures_new/splitMNIST_fisher_allinone0.3_noewc_new2.jpg}
\includegraphics[width=1\linewidth]{text/figures_new/files/fisher3.pdf}
\end{center}
\vspace{-10pt}
\caption{\small{Parameter importance on different tasks. The x-axis represents each different parameter and y-axis is the FIM value in \eqn{eqn:fisher}. The sparser the parameters are, the fewer important parameters for previous data, which may contribute to why EBMs has less influence on previous tasks after training on new data.
% the better the model is in learning new tasks with less influence on previous tasks. 
``Fisher 5 on data 1'' means the diagonal elements of the fisher information matrix obtained by \eqn{eqn:fisher} using the model parameters $\theta_5$ (after training on task $T_5$) and data from task $T_1$.}}
\label{fig:fisher}
\end{figure} 



==> text/figures_new/label_distributation.tex <==
\begin{wrapfigure}{R}{0.4\textwidth}
\begin{center}
\includegraphics[width=0.36\textwidth]{text/figures_new/files/split_label_distributation2.pdf}
\end{center}
\vspace{-12pt}
\caption{\small{Predicted label distribution after learning each task on the split MNIST dataset. The SBC only predicts classes from the current task, while our EBM predicts classes for all seen classes.}
%   The more uniform the distribution is, the better the model is in preventing forgetting previous tasks.
}
\label{fig:new_label_distributation}
\vspace{-15pt}
\end{wrapfigure} 

==> text/figures_new/landmap.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[width=0.3\textwidth]{text/figures_new/files/energy_landmap.pdf}
\end{center}
\vspace{-10pt}
\caption{\small{Energy landmaps of SBC and EBMs after training on task $T_9$ and $T_{10}$ on permuted MNIST. The darker the diagonal is, the better the model is in preventing forgetting previous tasks.}}
\label{fig:energy_landmap}
\vspace{-12pt}
\end{figure}




==> text/figures_new/training_curve.tex <==
% \begin{figure*}
% \begin{center}
% \includegraphics[width=1\linewidth]{text/figures_new/files/training_curve4.pdf}
% \end{center}
% \vspace{-15pt}
% \caption{\small{\emph{Class-IL} testing accuracy of the standard classifier (SBC) used in existing CL works, classifier using our training objective (SBC*), and EBMs on each task on the split MNIST dataset (left) and permuted MNIST dataset (right).}}
% \vspace{-10pt}
% \label{fig:training_curve}
% \end{figure*}


\begin{figure}[t]
\begin{center}
\includegraphics[width=1\linewidth]{text/figures_new/files/training_curve5.pdf}
\end{center}
\vspace{-15pt}
\caption{\small{\emph{Class-IL} testing accuracy of the standard classifier (SBC), classifier using our training objective (SBC*), and EBMs on each task on the permuted MNIST dataset.}}
\vspace{-10pt}
\label{fig:training_curve}
\end{figure}

==> text/figures_new/training_curve_landmap.tex <==
\begin{figure}[h]
     \centering
     \begin{minipage}[b]{0.39\textwidth}
         \centering
         \includegraphics[width=1\textwidth]{text/figures_new/files/training_curve.pdf}
         \caption{\small Class-IL testing accuracy of the standard classifier (CLS) and EBM on each task on the permuted MNIST.
        }
        \label{fig:new_training_curve}
     \end{minipage}
     \hfill
     \begin{minipage}[b]{0.59\textwidth}
         \centering
         \includegraphics[width=1\textwidth]{text/figures_new/files/landmap.pdf}
        \caption{\small Energy landmaps of CLS and EBM after training on task $T_9$ and $T_9$ on the permuted MNIST dataset.
        The darker the diagonal is, the better the model is in preventing forgetting previous tasks.}
        \label{fig:new_landmap}
    \end{minipage}
\end{figure}

==> text/tables_new/ablation.tex <==
% \begin{wraptable}{R}{0.38\textwidth}
% \vspace{-10pt}
%   \caption{\small{Performance of EBM on CIFAR-10 with different label conditioning architectures.}}
%   \vspace{-5pt}
%   \small
%   \label{tab:diff_net}
%   \centering
%   \scalebox{0.9}{
%   \begin{tabular}{lccc}
%     \toprule
%     \bf Dataset & \bf CIFAR-10 \\
%     \midrule
%     % \midrule
%     Beginning (V1) & 13.69 $\pm$ 1.12 \\ 
%     Middle(V2) & 20.16 $\pm$ 1.05 \\ 
%     Middle(V3) & 18.36 $\pm$ 0.97 \\
%     \bf End (V4) & 38.13 $\pm$ 0.59 \\
%     \midrule
%     End Fix (V4) & 34.30 $\pm$ 1.03 \\
%     End Fix Norm2 (V4) & 33.91 $\pm$ 1.13 \\
%     End Fix Softmax (V4) & 35.97 $\pm$ 1.09 \\
%     End Norm2 (V4) & 37.23 $\pm$ 1.20 \\ 
%     \bf End Softmax (V4) & \bf 38.84 $\pm$ 1.08 \\ 
%     \bottomrule
%   \end{tabular}
%   }
% \vspace{-10pt}
% \end{wraptable}




\begin{table}[t]
  \caption{\small{Performance of EBM on CIFAR-10 with different label conditioning architectures.}}
  \small
  \label{tab:diff_net}
  \centering
  \setlength{\tabcolsep}{3pt}
  \scalebox{0.9}{
  \begin{tabular}{lc|lc}
    \toprule
    \multicolumn{2}{c}{\bf Model architectures} & \multicolumn{2}{c}{\bf Normalization types} \\
    \midrule
    % \midrule
    Beginning (V1) & 13.69 $\pm$ 1.12 & End Fix (V4) & 34.30 $\pm$ 1.03 \\ 
    Middle(V2) & 20.16 $\pm$ 1.05 & End Fix Norm2 (V4) & 33.91 $\pm$ 1.13 \\ 
    Middle(V3) & 18.36 $\pm$ 0.97 & End Fix Softmax (V4) & 35.97 $\pm$ 1.09 \\
    \bf End (V4) & 38.13 $\pm$ 0.59 & End Norm2 (V4) & 37.23 $\pm$ 1.20 \\
    && \bf End Softmax (V4) & \bf 38.84 $\pm$ 1.08 \\
    \bottomrule
  \end{tabular}
  }
\vspace{-20pt}
\end{table}



==> text/tables_new/diff_num_tasks.tex <==
\begin{wraptable}{R}{0.57\textwidth}
\vspace{-10pt}
\small
    \caption{\small Comparison of our EBM with baselines on different variants of the split CIFAR-100 protocol. % The CIFAR-100 dataset is split up into 5 tasks (= 20 classes per task), 10 tasks (= 10 classes per task), 20 tasks (= 5 classes per task) or 50 tasks (= 2 classes per task).
    Results of the \emph{Class-IL} performance on the \emph{boundary-aware} setting are reported.
    % after all tasks have been learned. 
    % Each experiment is run 10 times with different random seeds, results are reported as mean $\pm$ SEM.
    }
    \vspace{-10pt}
    \setlength{\tabcolsep}{4pt}
    \label{tab:number_of_tasks}
    \begin{center}
    \begin{small}
    \scalebox{0.85}{
    \begin{tabular}{lcccc}
    \toprule
    \multirow{2}{*}{\bf Method} & \multicolumn{4}{c}{\bf CIFAR-100 split up into:} \\
    & \bf 5 tasks & \bf 10 tasks & \bf 20 tasks & \bf 50 tasks \\
    \midrule
    SBC & 14.74 $\pm$ 0.20 & 8.18 $\pm$ 0.10 & 4.46 $\pm$ 0.03 & 1.91 $\pm$ 0.02 \\ 
    EWC & 14.78 $\pm$ 0.21 & 8.20 $\pm$ 0.09 & 4.46 $\pm$ 0.03 & 1.91 $\pm$ 0.02  \\
    SI & 14.07 $\pm$ 0.24 & 9.24 $\pm$ 0.22 & 4.37 $\pm$ 0.04 & 1.88 $\pm$ 0.03  \\
    LwF & 25.75 $\pm$ 0.14 & 10.71 $\pm$ 0.11 & 12.18 $\pm$ 0.16 & 7.68 $\pm$ 0.16  \\
    \midrule
    \bf EBM & \bf 34.88 $\pm$ 0.14 & \bf 30.28 $\pm$ 0.28 & \bf 25.04 $\pm$ 0.33 & \bf 13.60 $\pm$ 0.50  \\
    \bottomrule
    \end{tabular}
    }
    \end{small}
    \end{center}
\vspace{-10pt}
\end{wraptable}
    

==> text/tables_new/diff_num_tasks_replay.tex <==
\begin{table*}
\centering
\hfill
\begin{minipage}{0.37\textwidth}
    \caption{\small Comparisons of the softmax-based classifier and EBMs using exact replay on four datasets. Results of \emph{Class-IL} on the \emph{boundary-aware} setting are reported. $k$ is the memory budget size.}
    \vspace{-10pt}
    \small
    \label{tab:comp_baselines_boundary_aware_replay}
    \begin{center}
    \scalebox{0.83}{
    \begin{tabular}{lcc}
    \toprule
    \bf Dataset & \bf SBC ER & \bf EBM ER \\
    \midrule
    \midrule
    splitMNIST & 90.65 $\pm$ 0.45 & 91.13 $\pm$ 0.35 \\
    permMNIST & 93.70 $\pm$ 0.09 & 94.59 $\pm$ 0.09 \\
    CIFAR-10 & 42.07 $\pm$ 0.64 & 44.76 $\pm$ 0.73 \\
    CIFAR-100 & 28.57 $\pm$ 0.35 & 34.07 $\pm$ 0.55 \\
    \bottomrule
    \end{tabular}
    }
    \end{center}
    \end{minipage}%
    \hfill
    \hfill
    \begin{minipage}{0.58\textwidth}
    \caption{\small Comparison of our EBM with baselines on different variants of the split CIFAR-100 protocol. % The CIFAR-100 dataset is split up into 5 tasks (= 20 classes per task), 10 tasks (= 10 classes per task), 20 tasks (= 5 classes per task) or 50 tasks (= 2 classes per task).
    Results of the \emph{Class-IL} performance on the \emph{boundary-aware} setting are reported.
    % after all tasks have been learned. 
    % Each experiment is run 10 times with different random seeds, results are reported as mean $\pm$ SEM.
    }
    \vspace{-10pt}
    \setlength{\tabcolsep}{4pt}
    \label{tab:number_of_tasks}
    \begin{center}
    \begin{small}
    \scalebox{0.85}{
    \begin{tabular}{lcccc}
    \toprule
    \multirow{2}{*}{\bf Method} & \multicolumn{4}{c}{\bf CIFAR-100 split up into:} \\
    & \bf 5 tasks & \bf 10 tasks & \bf 20 tasks & \bf 50 tasks \\
    \midrule
    SBC & 14.74 $\pm$ 0.20 & 8.18 $\pm$ 0.10 & 4.46 $\pm$ 0.03 & 1.91 $\pm$ 0.02 \\ 
    EWC & 14.78 $\pm$ 0.21 & 8.20 $\pm$ 0.09 & 4.46 $\pm$ 0.03 & 1.91 $\pm$ 0.02  \\
    SI & 14.07 $\pm$ 0.24 & 9.24 $\pm$ 0.22 & 4.37 $\pm$ 0.04 & 1.88 $\pm$ 0.03  \\
    LwF & 25.75 $\pm$ 0.14 & 10.71 $\pm$ 0.11 & 12.18 $\pm$ 0.16 & 7.68 $\pm$ 0.16  \\
    \midrule
    \bf EBM & \bf 34.88 $\pm$ 0.14 & \bf 30.28 $\pm$ 0.28 & \bf 25.04 $\pm$ 0.33 & \bf 13.60 $\pm$ 0.50  \\
    \bottomrule
    \end{tabular}
    }
    \end{small}
    \end{center}
    \end{minipage}
\vspace{-10pt}
\end{table*}




==> text/tables_new/negative_sampling.tex <==
\begin{table}[t]
\small
  \caption{\small{Performance of EBM on CIFAR-100 with different strategies for selecting the negative samples.}}
  \label{tab:neg_sam}
  \centering
  \scalebox{0.9}{
  \begin{tabular}{lccc}
    \toprule
    \bf Dataset & \bf CIFAR-100 \\
    \midrule
    % \midrule
    All Neg Seen & 8.07 $\pm$ 0.10 \\
    All Neg Batch & 29.03 $\pm$ 0.53 \\
    \bf 1 Neg Batch & \bf 30.28 $\pm$ \bf 0.28 \\
    \bottomrule
  \end{tabular}
  }
\end{table}


==> text/tables_new/negative_sampling_training_objective.tex <==
\begin{table*}
\centering
\hfill
\begin{minipage}{0.3\textwidth}
    \centering
    \small
    \caption{\small{Performance of EBM on CIFAR-100 with different strategies for selecting the negative samples.}}
      \vspace{-3pt}
      \label{tab:neg_sam}
      \centering
      \scalebox{0.95}{
      \begin{tabular}{lccc}
        \toprule
        \bf Dataset & \bf CIFAR-100 \\
        \midrule
        \midrule
        All Neg Seen & 8.07 $\pm$ 0.10 \\
        All Neg Batch & 29.03 $\pm$ 0.53 \\
        \bf 1 Neg Batch & \bf 30.28 $\pm$ \bf 0.28 \\
        \bottomrule
      \end{tabular}
      }
    \label{tab:neg_sam}
    \end{minipage}%
    \hfill
    \begin{minipage}{0.65\textwidth}
    \centering
    \small
    \caption{\small Results of baselines using our training objective and their original one.}
    \vspace{-10pt}
    \label{tab:new_train_strategy}
    \scalebox{0.9}{
    \begin{tabular}{lcccc} 
        \toprule
         & \multicolumn{2}{c}{\bf split MNIST} & \multicolumn{2}{c}{\bf CIFAR-10} \\
         & Original & Ours & Original & Ours  \\
        \midrule
        \midrule
        SBC & 19.90 $\pm$ 0.02 & 44.98 $\pm$ 0.05 & 19.06 $\pm$ 0.01 & 19.22 $\pm$ 0.02 \\
        EWC & 20.01 $\pm$ 0.06 & 50.68 $\pm$ 0.04 & 18.99 $\pm$ 0.01 & 36.51 $\pm$ 0.03 \\
        Online EWC & 19.96 $\pm$ 0.07 & 50.99 $\pm$ 0.03 & 19.07 $\pm$ 0.01 & 36.16 $\pm$ 0.02 \\
        SI & 19.99 $\pm$ 0.06 & 49.44 $\pm$ 0.03 & 19.14 $\pm$ 0.02 & 35.12 $\pm$ 0.02 \\
        EBM & - & \bf 53.12 $\pm$ 0.04 & - & \bf 40.19 $\pm$ 0.01 \\
        \bottomrule
    \end{tabular}
    }
    \end{minipage}
\vspace{-10pt}
\end{table*}



% \begin{table}
% \small
%   \caption{\small{Performance of EBM on CIFAR-100 with different strategies for selecting the negative samples.}}
%   \vspace{-3pt}
%   \label{tab:neg_sam}
%   \centering
%   \begin{tabular}{lccc}
%     \toprule
%     \bf Dataset & \bf CIFAR-100 \\
%     \midrule
%     \midrule
%     All Neg Seen & 8.07 $\pm$ 0.10 \\
%     All Neg Batch & 29.03 $\pm$ 0.53 \\
%     \bf 1 Neg Batch & \bf 30.28 $\pm$ \bf 0.28 \\
%     \bottomrule
%   \end{tabular}
%   \vspace{-5pt}
% \end{table}





% \begin{table*}[t]
% \small
% \caption{\small Results of baselines using our training objective and their original one.}
% \vspace{-10pt}
% \label{tab:new_train_strategy}
% \begin{center}
% \scalebox{0.95}{
% \begin{tabular}{lcccc} 
%     \toprule
%      & \multicolumn{2}{c}{\bf split MNIST} & \multicolumn{2}{c}{\bf CIFAR-10} \\
%      & Original & Ours & Original & Ours  \\
%     \midrule
%     \midrule
%     SBC & 19.90 $\pm$ 0.02 & 44.98 $\pm$ 0.05 & 19.06 $\pm$ 0.01 & 19.22 $\pm$ 0.02 \\
%     EWC & 20.01 $\pm$ 0.06 & 50.68 $\pm$ 0.04 & 18.99 $\pm$ 0.01 & 36.51 $\pm$ 0.03 \\
%     Online EWC & 19.96 $\pm$ 0.07 & 50.99 $\pm$ 0.03 & 19.07 $\pm$ 0.01 & 36.16 $\pm$ 0.02 \\
%     SI & 19.99 $\pm$ 0.06 & 49.44 $\pm$ 0.03 & 19.14 $\pm$ 0.02 & 35.12 $\pm$ 0.02 \\
%     EBM & - & \bf 53.12 $\pm$ 0.04 & - & \bf 40.19 $\pm$ 0.01 \\
%     \bottomrule
% \end{tabular}
% }
% \end{center}
% \end{table*}

==> text/tables_new/replay.tex <==
\begin{table}[t]
\vspace{-3pt}
    \caption{\small Comparisons of the softmax-based classifier and EBMs using exact replay on four datasets. Results of \emph{Class-IL} on the \emph{boundary-aware} setting are reported. $k$ is the memory budget size.}
    \small
    \label{tab:comp_baselines_boundary_aware_replay}
    \begin{center}
    \scalebox{0.82}{
    \begin{tabular}{lcccc}
    \toprule
    \bf Method & \bf splitMNIST & \bf permMNIST & \bf CIFAR-10 & \bf CIFAR-100 \\
    \midrule
    & k=1000 & k=1000 & k=1000 & k=2000 \\
    \midrule
    % A-GEM & 66.27 $\pm$ 3.48 & 90.54 $\pm$ 0.18 & 18.81 $\pm$ 0.41 & 11.32 $\pm$ 0.52 \\
    % GR & 91.20 $\pm$ 0.39 & 92.37 $\pm$ 0.10 & & - \\
    % iCaRL & 93.53 $\pm$ 0.12 & 94.00 $\pm$ 0.07 && 35.31 $\pm$ 0.28  \\
    SBC ER & 90.65 $\pm$ 0.45 & 93.70 $\pm$ 0.09 & 42.07 $\pm$ 0.64 & 28.57 $\pm$ 0.35 \\
    EBM ER & 91.13 $\pm$ 0.35 & 94.59 $\pm$ 0.09 & 44.76 $\pm$ 0.73 & 34.07 $\pm$ 0.55 \\
    \bottomrule
    \end{tabular}
    }
    \end{center}
\vspace{-20pt}
\end{table}




==> text/tables_new/training_curve.tex <==

\begin{wrapfigure}{r}{0.6\textwidth}
\vspace{-10pt}
  \begin{center}
    \includegraphics[width=1\linewidth]{text/figures_new/files/training_curve5.pdf}
  \end{center}
  \vspace{-10pt}
  \caption{\small{\emph{Class-IL} testing accuracy of SBC, SBC using our training objective (SBC*), and EBMs on each task on permuted MNIST.}}
    \label{fig:training_curve}
\end{wrapfigure}


==> text/tables_new/training_objective.tex <==
\begin{table}[t]
\small
\caption{\small Continual learning approaches using our training objective and their original one.}
\label{tab:new_train_strategy}
\begin{center}
\setlength{\tabcolsep}{4pt}
\scalebox{0.82}{
\begin{tabular}{lcccc} 
    \toprule
     & \multicolumn{2}{c}{\bf split MNIST} & \multicolumn{2}{c}{\bf CIFAR-10} \\
     & Original & Ours & Original & Ours  \\
    \midrule
    % \midrule
    SBC & 19.90 $\pm$ 0.02 & 44.98 $\pm$ 0.05 & 19.06 $\pm$ 0.05 & 19.22 $\pm$ 1.12 \\
    EWC & 20.01 $\pm$ 0.06 & 50.68 $\pm$ 0.04 & 18.99 $\pm$ 0.03 & 36.51 $\pm$ 1.20 \\
    Online EWC & 19.96 $\pm$ 0.07 & 50.99 $\pm$ 0.03 & 19.07 $\pm$ 0.13 & 36.16 $\pm$ 1.02 \\
    SI & 19.99 $\pm$ 0.06 & 49.44 $\pm$ 0.03 & 19.14 $\pm$ 0.12 & 35.12 $\pm$ 1.70 \\
    EBM & - & \bf 53.12 $\pm$ 0.04 & - & \bf 38.84 $\pm$ 1.08 \\
    \bottomrule
\end{tabular}
}
\end{center}
\vspace{-15pt}
\end{table}




==> text/tables_new/var_num_class.tex <==
\begin{table}
  \small
  \caption{\small{CL.}}
  \label{tab:comp_baselines_var_num}
  \centering
  \resizebox{1\textwidth}{!}{
  \begin{tabular}{lccc|ccc}
    \toprule
    % \multirow{2}*{\bf Metric}    
    & \multicolumn{3}{c|}{\bf No overlap between tasks} & \multicolumn{3}{c}{\bf Overlap between tasks} \\
    \bf Dataset & \bf MNIST & \bf Cifar10 & \bf Cifar100 & \bf MNIST & \bf Cifar10 & \bf Cifar100  \\
    \midrule
    \midrule
    CLS &  \\ 
    CLS+EWC &  \\
    CLS+Online & \\
    CLS+SI & \\
    LwF &  \\
    MAS &  \\
    BGD &  \\
    CLS* &  \\
    \midrule
    \bf EBM & \\
    \bottomrule
  \end{tabular}
  }
\vspace{-10pt}
\end{table}



